Multi-dimensional Approximate Counting

The celebrated Morris counter uses $\log_2\log_2 n + O(\log_2 \sigma^{-1})$ bits to count up to $n$ with a relative error $\sigma$, where if $\hat{\lambda}$ is the estimate of the current count $\lambda$, then $\mathbb{E}|\hat{\lambda}-\lambda|^2 <\sigma^2\lambda^2$. A natural generalization is \emph{multi-dimensional} approximate counting. Let $d\geq 1$ be the dimension. The count vector $x\in \mathbb{N}^d$ is incremented entry-wisely over a stream of coordinates $(w_1,\ldots,w_n)\in [d]^n$, where upon receiving $w_k\in[d]$, $x_{w_k}\gets x_{w_k}+1$. A \emph{$d$-dimensional approximate counter} is required to count $d$ coordinates simultaneously and return an estimate $\hat{x}$ of the count vector $x$. Aden-Ali, Han, Nelson, and Yu \cite{aden2022amortized} showed that the trivial solution of using $d$ Morris counters that track $d$ coordinates separately is already optimal in space, \emph{if each entry only allows error relative to itself}, i.e., $\mathbb{E}|\hat{x}_j-x_j|^2<\sigma^2|x_j|^2$ for each $j\in [d]$. However, for another natural error metric -- the \emph{Euclidean mean squared error} $\mathbb{E} |\hat{x}-x|^2$ -- we show that using $d$ separate Morris counters is sub-optimal. In this work, we present a simple and optimal $d$-dimensional counter with Euclidean relative error $\sigma$, i.e., $\mathbb{E} |\hat{x}-x|^2 <\sigma^2|x|^2$ where $|x|=\sqrt{\sum_{j=1}^d x_j^2}$, with a matching lower bound. The upper and lower bounds are proved with ideas that are strikingly simple. The upper bound is constructed with a certain variable-length integer encoding and the lower bound is derived from a straightforward volumetric estimation of sphere covering.

==> pool.tex <==
\section{}

The multiplicative covering corresponds to the \emph{offline} version of approximate counting, for which one only needs to construct a set of ``answers'' $R$ such that for any ``question'' $x$ in $A$, there exists $y\in R$ such that $|x-y|<\sigma|x|$. The offline version surely uses less space in comparison to the online version which tracks the target over an incremental stream. 
 It is not hard to see that it needs at least $\log_{1+\sigma} n \geq  \sigma^{-1}\log n$ points to $\sigma$-multiplicatively cover $\{0,1,\ldots,n\}$. 
 Therefore, the memory space needed to encode the covering is $\log_2\log_2 n +\Omega(\log \sigma^{-1})$, which matches the space of Morris counter $\log_2\log_2 n +O(\log_2\sigma^{-1})$. In other words, the Morris counter suggests that the 1-dimensional approximate counting has the same space complexity for the offline and online settings. Similarly, the lower bound in \cref{thm:main} is derived by estimating the size of the covering needed to cover $\{x\in\N^d|x_1+\ldots +x_d \leq n\}$. It turns out that $d$-dimensional counting with $d\geq 2$ also has a matching complexity for the offline and online settings, which is $\log_2\log_2 n + O(d\log_2\sigma^{-1})$.

\section{}


The intuition is that, the \emph{discretization error} of the representation will grow as the dimension $d$ increases and thus $m$ has to depend on $d$.  To see this, we assume $\sigma$ is a fixed constant and consider $d$ $\mathrm{Morris}(a)$ counters with $a=O(\sigma^{-2})$. By \cref{def:morris}, the  estimate given by $\mathrm{Morris}(a)$ with index $r$ is $a((1+1/a)^{r}-1)\approx a(1+1/a)^{r}$ when $r\gg 1$. Now suppose the is input count vector is $a\left((1+1/a)^{m+s},\frac{1}{2}(1+1/a)^s,\ldots,\frac{1}{2}(1+1/a)^s\right)$. The first entry $U+Z_1$ is thus around $m+s$ while the other entries $U+Z_2,\ldots,U+Z_d$ \emph{should} be around $s-\log_{1+1/a}2\approx s-2a$ but cannot be represented since $Z_j$s are only allowed to be in $[0,m]$. To work around this, when $Z_j$ needs to be negative, one may probabilistic round the index $U+Z_j$ to either $U$ or a special state $\perp$ that returns 0 as the estimate. In such a way, unbiasedness can be maintained but the mean squared error for estimating $x$ is now at least $\frac{d-1}{4}a^2(1+1/a)^{2s}$ with $|x|^2=a^2(1+1/a)^{2s}((1+1/a)^{2m}+\frac{d-1}{4})$. Thus for a relative error $\sigma$, one needs $\frac{d-1}{4}a^2(1+1/a)^{2s}<\sigma^2 |x|^2$, which implies $2m\log (1+1/a)>\log ((d-1)/4)+\log(\sigma^{-2}-1)$, i.e., $m=\Omega(\sigma^{-2}\log d)$. Thus this strategy needs, at the very least, $\Omega(d\log\sigma^{-1}+d\log\log d)$ bits with the rough estimate above.

\section{}
We consider the case where $r\gg 1$ and approximate $a((1+1/a)^{r}-1)\approx a(1+1/a)^r$ for simplicity. Thus given the $d$ indices $(U+V_1,U+V_2,\ldots,U+V_d)$, the estimate for the vector is $\hat{x}=a(1+1/a)^U((1+1/a)^{V_1},(1+1/a)^{V_2},\ldots,(1+1/a)^{V_d})$. Suppose now we have the input count vector
\begin{align*}
    x = a(1+1/a)^s\left((1+1/a)^{m},\frac{1}{2}(1+1/a),\ldots,\frac{1}{2}(1+1/a)\right),
\end{align*}
where by construction
\begin{align*}
\left|\hat{x}-x\right|^2&= a^2\left(((1+1/a)^{U+V_1}-(1+1/a)^{s+m})^2+\sum_{j=2}^d((1+1/a)^{U+V_j}-(1+1/a)^{s}/2)^2\right)\\
&\geq a^2\left(((1+1/a)^{U+m}-(1+1/a)^{s+m})^2+\sum_{j=2}^d((1+1/a)^{U}-(1+1/a)^{s}/2)^2\right)\\
&\geq a^2(1+1/a)^{2s}\left((1+1/a)^{2m}((1+1/a)^{U-s}-1)^2+(d-1)((1+1/a)^{U-s}-1/2)^2\right)
\end{align*}
